Measurement of the Bottom-Strange Meson Mixing Phase in the Full CDF Data Set

We report a measurement of the bottom-strange meson mixing phase \beta_s using the time evolution of B0_s -> J/\psi (->\mu+\mu-) \phi (-> K+ K-) decays in which the quark-flavor content of the bottom-strange meson is identified at production. This measurement uses the full data set of proton-antiproton collisions at sqrt(s)= 1.96 TeV collected by the Collider Detector experiment at the Fermilab Tevatron, corresponding to 9.6 fb-1 of integrated luminosity. We report confidence regions in the two-dimensional space of \beta_s and the B0_s decay-width difference \Delta\Gamma_s, and measure \beta_s in [-\pi/2, -1.51] U [-0.06, 0.30] U [1.26, \pi/2] at the 68% confidence level, in agreement with the standard model expectation. Assuming the standard model value of \beta_s, we also determine \Delta\Gamma_s = 0.068 +- 0.026 (stat) +- 0.009 (syst) ps-1 and the mean B0_s lifetime, \tau_s = 1.528 +- 0.019 (stat) +- 0.009 (syst) ps, which are consistent and competitive with determinations by other experiments.

==> macro.tex <==

\newcommand{\Acp}{\ensuremath{A_\textit{CP}}}
\newcommand{\Acpraw}{\ensuremath{\Acp^{\text{raw}}}}
\newcommand{\acp}[1]{\ensuremath{a_{\text{CP}}^{\text{#1}}}}
\newcommand{\stat}{\ensuremath{\mathrm{~(stat)}}}
\newcommand{\syst}{\ensuremath{\mathrm{~(syst)}}}
\newcommand{\Dbar}{\ensuremath{\overline{D}{}}}
\newcommand{\Dhh}{\ensuremath{D^0\to h^+h'^-}}


%%%%%%%%%%%%%%%  GENERAL JARGON  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \rightdownarrow
 {\kern.3em
 \rule[.5ex]{.15mm}{2ex}
 {\mbox{$\kern-0.1em{\longrightarrow}$}}      % down-right arrow for cascade decay equations
 }

 
\def\lessim{\mathrel {\vcenter {\baselineskip 0pt \kern 0pt  % minore/circa uguale
\hbox{$<$} \kern 0pt \hbox{$\sim$} }}}


\def\gessim{\mathrel {\vcenter {\baselineskip 0pt \kern 0pt   % maggiore/circa uguale
\hbox{$>$} \kern 0pt \hbox{$\sim$} }}}


\newcommand{\ie}{i.~e.,}					%   	cioe' 
\newcommand{\eg}{e.~g.,}					%   	per esempio 
\newcommand{\etc}{etc.}
\newcommand{\st}{\ensuremath{\mathrm{st}}}
\newcommand{\nd}{\ensuremath{\mathrm{nd}}}
\newcommand{\rd}{\ensuremath{\mathrm{rd}}}
\newcommand{\jth}{\ensuremath{\mathrm{th}}}

\newcommand{\pipi}{\ensuremath{\pi^+\pi^-}}
\newcommand{\KK}{\ensuremath{K^+K^-}}
\newcommand{\Kpi}{\ensuremath{K^+\pi^-}}
\newcommand{\piK}{\ensuremath{K^-\pi^+}}

\newcommand{\mpipi}{\ensuremath{m_{\pipi}}}
\newcommand{\mKK}{\ensuremath{m_{\KK}}}
\newcommand{\mKpi}{\ensuremath{m_{\Kpi}}}
\newcommand{\mpiK}{\ensuremath{m_{\piK}}}
\newcommand{\mDKpi}{\ensuremath{m_{K^-\pi^+}}}
\newcommand{\maDKpi}{\ensuremath{m_{K^+\pi^-}}}



\newcommand{\babelle}{\mbox{$B$-Factories}}

\newcommand{\lumi}{\mbox{cm$^{-2}$s$^{-1}$}}  	 		%	cm^-2 s^-1
\newcommand{\Lumi}{\ensuremath{\mathcal{L}}}			%	L maiuscola di luminosita' istantanea
\newcommand{\intlumi}{\ensuremath{\int\Lumi dt}}
\newcommand{\luminb}{\mbox{nb$^{-1}$}}
\newcommand{\lumipb}{\mbox{pb$^{-1}$}}				%	pb^-1
\newcommand{\lumifb}{\mbox{fb$^{-1}$}}				%	fb^-1

\newcommand{\ecm}{\ensuremath{\sqrt{s}}}

\newcommand{\boost}{\ensuremath{\beta\gamma}}
\newcommand{\vecboost}{\ensuremath{\vec{\beta}\gamma}}
\newcommand{\tboost}{\ensuremath{\beta_{\rm{T}}\gamma}}
\newcommand{\vectboost}{\ensuremath{\vec{\beta}_{\rm{T}}\gamma}}
\newcommand{\mum}{\mbox{$\mu$m}}				%	um
\newcommand{\mus}{\mbox{$\mu$s}}

\newcommand{\sm}{\mbox{Standard Model}}
\newcommand{\np}{\mbox{New Physics}}
\newcommand{\SUtre}{\mbox{SU(3)}}
\newcommand{\SUdue}{\mbox{SU(2)}}
\newcommand{\Uspin}{\mbox{U-spin}}
\newcommand{\Uuno}{\mbox{U(1)}}
\newcommand{\Rds}{\ensuremath{R_d^s}}

\newcommand{\br}{\ensuremath{\mathcal{B}}}
\newcommand{\amp}{\ensuremath{\mathcal{A}}}
\newcommand{\vmau}{\ensuremath{\gamma^\mu(1-\gamma_5)}}
\newcommand{\vmad}{\ensuremath{\gamma_\mu(1-\gamma_5)}}
\newcommand{\vpau}{\ensuremath{\gamma^\mu(1+\gamma_5)}}
\newcommand{\vpad}{\ensuremath{\gamma_\mu(1+\gamma_5)}}



\newcommand{\tev}{\ensuremath{\mathrm{Te\kern -0.1em V}}}
\newcommand{\gev}{\ensuremath{\mathrm{Ge\kern -0.1em V}}}	%	GeV
\newcommand{\mev}{\ensuremath{\mathrm{Me\kern -0.1em V}}}	%	MeV
\newcommand{\kev}{\ensuremath{\mathrm{ke\kern -0.1em V}}}	%	keV
\newcommand{\massgev}{\mbox{\gev/$c^2$}}			%	GeV/c^2
\newcommand{\massmev}{\mbox{\mev/$c^2$}}			%	MeV/c^2
\newcommand{\pgev}{\mbox{\gev/$c$}}				%	GeV/c
\newcommand{\pmev}{\mbox{\mev/$c$}}				%	MeV/c

\newcommand{\sye}[1]{\ensuremath{\pm #1}}	   		%	+/- X
\newcommand{\ase}[2]{\ensuremath{^{+ #1}_{- #2}}}		%	+X 
								%	-Y

\newcommand{\TTT}{Displaced-Tracks Trigger}
\newcommand{\TTTs}{Displaced-Tracks Triggers}
\newcommand{\bcharm}{\texttt{B\_CHARM}}
\newcommand{\bcharmlowpt}{\texttt{B\_CHARM\_LOWPT}}
\newcommand{\bcharmhighpt}{\texttt{B\_CHARM\_HIGHPT}}
\newcommand{\bpipi}{\texttt{B\_PIPI}}
\newcommand{\bpipihighpt}{\texttt{B\_PIPI\_HIGHPT}}
\newcommand{\bpipilowpt}{\texttt{B\_PIPI\_LOWPT}}

\newcommand{\svxii}{\ensuremath{\rm{SVXII}}}



%%%%%%%%%%%%%%% CP PHYSICS %%%%%%%%%%%%%%%%%

\newcommand{\CPV}{\ensuremath{\mathsf{C\!P}}}			%	CP barrato
\newcommand{\MET}{\ensuremath{\mathsf{E\!_{T}}}}			%	CP barrato
%\newcommand{\CP}{\ensuremath{\mathsf{CP}}}			%	CP
\newcommand{\CP}{{\it CP}}                                            %	CP
\newcommand{\Charge}{\ensuremath{\mathsf{C}}}
\newcommand{\Parity}{\ensuremath{\mathsf{P}}}
\newcommand{\Time}{\ensuremath{\mathsf{T}}}
\newcommand{\CPT}{\ensuremath{\mathsf{CPT}}}
					
\newcommand{\vij}{\ensuremath{V_{ij}}}				%	CKM elements
\newcommand{\vud}{\ensuremath{V_{ud}}}
\newcommand{\vus}{\ensuremath{V_{us}}}
\newcommand{\vub}{\ensuremath{V_{ub}}}
\newcommand{\vcd}{\ensuremath{V_{cd}}}
\newcommand{\vcs}{\ensuremath{V_{cs}}}
\newcommand{\vcb}{\ensuremath{V_{cb}}}
\newcommand{\vtd}{\ensuremath{V_{td}}}
\newcommand{\vts}{\ensuremath{V_{ts}}}
\newcommand{\vtb}{\ensuremath{V_{tb}}}
\newcommand{\vckm}{\boldmath\ensuremath{V_{\rm{CKM}}}\unboldmath}

\newcommand{\apc}{\ensuremath{\amp_{\mathcal{P}}^{c}}}
\newcommand{\apt}{\ensuremath{\amp_{\mathcal{P}}^{t}}}
\newcommand{\apu}{\ensuremath{\amp_{\mathcal{P}}^{u}}}
\newcommand{\atu}{\ensuremath{\amp_{\mathcal{T}}^{u}}}

\newcommand{\apcp}{\ensuremath{\amp_{\mathcal{P}}^{\prime c}}}
\newcommand{\aptp}{\ensuremath{\amp_{\mathcal{P}}^{\prime t}}}
\newcommand{\apup}{\ensuremath{\amp_{\mathcal{P}}^{\prime u}}}
\newcommand{\atup}{\ensuremath{\amp_{\mathcal{T}}^{\prime u}}}


\newcommand{\rhobar}{\ensuremath{\bar{\rho}}}
\newcommand{\etabar}{\ensuremath{\bar{\eta}}}

\newcommand{\parc}{\ensuremath{\mathcal{C}}}
\newcommand{\parcprime}{\ensuremath{\mathcal{C'}}}



%%%%%%%%%% COLLIDER PHYSICS %%%%%%%%%

\newcommand{\pap}{\proton\antiproton}			%	ppbar
\newcommand{\pt}{\ensuremath{p_{\rm{T}}}}			%	pT
\newcommand{\vecpt}{\ensuremath{\vec{p}_{\rm{T}}}}
\newcommand{\ptb}{\ensuremath{\pt(B)}}				%	pT(B)
\newcommand{\vecptb}{\ensuremath{\vec{p}_{\rm{T}}(B)}}
\newcommand{\ptbd}{\ensuremath{\pt(\bd)}}			%	pT(B^0)
\newcommand{\ptbs}{\ensuremath{\pt(\bs)}}			%	pT(B^0_s)

\newcommand{\etad}{\ensuremath{\eta_{\rm{det}}}}
\newcommand{\Et}{\ensuremath{E_{\rm{T}}}}

%\newcommand{\lxy}{\ensuremath{L_{xy}}}	  
%\newcommand{\lxyb}{\ensuremath{L_{xy}(B)}}

\newcommand{\lxy}{\ensuremath{L_{\rm{T}}}}	  
\newcommand{\lxyb}{\ensuremath{L_{\rm{T}}(B)}}

%%%%%%%%%%%%%% CDF DETECTOR & SOFTWARE %%%%%%%%%%%

\newcommand{\cdfii}{CDF II}
\newcommand{\runi}{Run I}
\newcommand{\runii}{Run II}
\newcommand{\Loo}{L\O\O}
\newcommand{\geant}{{\scshape geant}}				%	GEANT	 
\newcommand{\DO}{D\0}

\newcommand{\gflash}{{\scshape gflash}} 
\newcommand{\garfield}{{\scshape garfield}}
\newcommand{\bgen}{{\scshape bgenerator}}			% 	BGENERATOR
\newcommand{\evtgen}{{\scshape evtgen}}
\newcommand{\pythia}{{\scshape pythia}}				%	PYTHIA     
\newcommand{\ctvmft}{{\scshape ctvmft}}
\newcommand{\photos}{{\scshape photos}}

\newcommand{\Lone}{Level-1}
\newcommand{\Ltwo}{Level-2}
\newcommand{\Lthree}{Level-3}

\newcommand{\minuit}{{\scshape minuit}}				%	MINUIT	  
\newcommand{\migrad}{{\scshape migrad}}				% 	MIGRAD
\newcommand{\minos}{{\scshape minos}}
\newcommand{\hesse}{{\scshape hesse}}
\newcommand{\mncontour}{{\scshape mncontour}}
\newcommand{\mathematica}{{\scshape mathematica$^{\rm{TM}}$}}		%	MATHEMATICA    
\newcommand{\ranlux}{{\scshape ranlux}}
\newcommand{\linux}{{\scshape linux}}
\newcommand{\gcc}{{\scshape gcc}}
\newcommand{\clanguage}{{\scshape c}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   	 PDG    %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\proton}{\ensuremath{\mathrm{p}}}
%\newcommand{\antiproton}{\ensuremath{\bar{\rm{p}}}}
%\newcommand{\electron}{\ensuremath{\rm{e}^-}}
%\newcommand{\positron}{\ensuremath{\rm{e}^+}}


\newcommand{\proton}{\ensuremath{p}}
\newcommand{\antiproton}{\ensuremath{\bar{p}}}
\newcommand{\electron}{\ensuremath{e^-}}
\newcommand{\positron}{\ensuremath{e^+}}


\newcommand{\lambdazero}{\ensuremath{\Lambda^0}}
\newcommand{\lambdazeroppi}{\ensuremath{\lambdazero \to \proton \pi^-}}


%%%%%%%%%%%%%%%%%  	BEAUTY  %%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bab}{\ensuremath{b\bar{b}}}

		%** hadrons **%

\newcommand{\Y}{\ensuremath{\Upsilon}}
\newcommand{\Yunos}{\mbox{$\Upsilon$(1S)}}
\newcommand{\Ydues}{\mbox{$\Upsilon$(2S)}}
\newcommand{\Ytres}{\mbox{$\Upsilon$(3S)}}
\newcommand{\Yquattros}{\mbox{$\Upsilon$(4S)}}
\newcommand{\Ycinques}{\mbox{$\Upsilon$(5S)}}
\newcommand{\BAB}{\ensuremath{B\overline{B}}}
\newcommand{\Ks}{\ensuremath{K^0_S}}
\newcommand{\Kl}{\ensuremath{K^0_L}}


\newcommand{\bd}{\ensuremath{B^{0}}}				% 	B-zero
\newcommand{\bs}{\ensuremath{B^{0}_s}}				% 	B (zero) sub-s


\newcommand{\bsshort}{\ensuremath{B^{0}_{s,\rm{short}}}}
\newcommand{\bslong}{\ensuremath{B^{0}_{s,\rm{long}}}}
\newcommand{\bseven}{\ensuremath{B^{0}_{s,\rm{even}}}}
\newcommand{\bsodd}{\ensuremath{B^{0}_{s,\rm{odd}}}}
\newcommand{\bsheavy}{\ensuremath{B^{0}_{s,H}}}
\newcommand{\bslight}{\ensuremath{B^{0}_{s,L}}}

\newcommand{\bq}{\ensuremath{B^{0}_{q}}}
\newcommand{\abq}{\ensuremath{\overline{B}^{0}_{q}}}
\newcommand{\bqpm}{\ensuremath{B^{0}_{q,\pm}}}
\newcommand{\bqp}{\ensuremath{B^{0}_{q,+}}}
\newcommand{\bqm}{\ensuremath{B^{0}_{q,-}}}
\newcommand{\lqpm}{\ensuremath{\lambda_{q,\pm}}}
\newcommand{\lqp}{\ensuremath{\lambda_{q,+}}}
\newcommand{\lqm}{\ensuremath{\lambda_{q,-}}}


\newcommand{\Mq}{\ensuremath{M^{(q)}}}
\newcommand{\Mqs}{\ensuremath{M^{(q)*}}}
\newcommand{\Gq}{\ensuremath{\Gamma^{(q)}}}
\newcommand{\Gqs}{\ensuremath{\Gamma^{(q)*}}}
\newcommand{\Tq}{\ensuremath{\Theta^{(q)}}}
\newcommand{\ham}{\ensuremath{\mathcal{H}}}
\newcommand{\fqp}{\ensuremath{f^{(q)}_{+}}}
\newcommand{\fqm}{\ensuremath{f^{(q)}_{-}}}
\newcommand{\fqpm}{\ensuremath{f^{(q)}_{\pm}}}
\newcommand{\gqp}{\ensuremath{g^{(q)}_{+}(t)}}
\newcommand{\gqm}{\ensuremath{g^{(q)}_{-}(t)}}
\newcommand{\gqpm}{\ensuremath{g^{(q)}_{\pm}(t)}}
\newcommand{\gqps}{\ensuremath{g^{(q)*}_{+}(t)}}
\newcommand{\gqms}{\ensuremath{g^{(q)*}_{-}(t)}}

\newcommand{\Dgq}{\ensuremath{\Delta\Gamma_q}}


\newcommand{\bu}{\ensuremath{B^{+}}}				%	B piu'
\newcommand{\bc}{\ensuremath{B^{+}_c}}				%	B sub-c (piu')

\newcommand{\abd}{\ensuremath{\overline{B}^{0}}}		% 	B-zero
\newcommand{\abs}{\ensuremath{\overline{B}^{0}_s}}		% 	B (zero) sub-s
\newcommand{\abu}{\ensuremath{B^{-}}}				%	B meno
\newcommand{\abc}{\ensuremath{B^{-}_c}}				%	B sub-c (meno)
	
\newcommand{\bphysics}{\mbox{$b$-physics}}

\newcommand{\bflavor}{\mbox{$b$-flavor}}			%	b-flavor	
\newcommand{\blavors}{\mbox{$b$-flavors}}			%	b-flavors
										
\newcommand{\bquark}{\mbox{$b$-quark}}				%	b-quark	
\newcommand{\bquarks}{\mbox{$b$-quarks}}			%	b-quarks

\newcommand{\bhadron}{\mbox{$b$-hadron}}			%	b-hadron
\newcommand{\bhadrons}{\mbox{$b$-hadrons}}			%	b-hadrons

\newcommand{\bbaryon}{\mbox{$b$-baryon}}			%	b-baryon
\newcommand{\bbaryons}{\mbox{$b$-baryons}}			%	b-baryons

\newcommand{\bg}{\ensuremath{B}}				% 	generic B
\newcommand{\bgmeson}{\mbox{$b$-meson}}				% 	generic B
\newcommand{\bgmesons}{\mbox{$b$-mesons}}			% 	generic B

\newcommand{\bn}{\ensuremath{B^{0}_{(s)}}}			% 	neutral B (B-zero and B sub-s)
\newcommand{\bnmeson}{\mbox{$B^0_{(s)}$ meson}}			% 	neutral B (B-zero and B sub-s)
\newcommand{\bnmesons}{\mbox{$B^0_{(s)}$ mesons}}		% 	neutral B (B-zero and B sub-s)

\newcommand{\abn}{\ensuremath{\overline{B}^{0}_{(s)}}}
\newcommand{\abnmeson}{\mbox{$\overline{B}^0_{(s)}$ meson}}			% 	neutral B (B-zero and B sub-s)
\newcommand{\abnmesons}{\mbox{$\overline{B}^0_{(s)}$ mesons}}	

\newcommand{\bdmeson}{\mbox{$B^0$ meson}}
\newcommand{\bsmeson}{\mbox{$B^0_{s}$ meson}}

\newcommand{\lambdab}{\ensuremath{\Lambda^0_{b}}}
\newcommand{\lambdabbaryon}{\mbox{$\Lambda^0_{b}$ baryon}}



%	** decays **

\newcommand{\bhh}{\ensuremath{\bn \to h^{+}h^{'-}}}
\newcommand{\fullbhh}{\ensuremath{B \to hh'}}
\newcommand{\sbhh}{\ensuremath{\bn \to h^{+}h^{-}}}

\newcommand{\bdpipi}{\ensuremath{\bd \to \pi^+ \pi^-}}
\newcommand{\abdpipi}{\ensuremath{\abd \to \pi^+ \pi^-}}
\newcommand{\bothbdpipi}{\ensuremath{\bd, \abd \to \pi^+ \pi^-}}

\newcommand{\bdkpi}{\ensuremath{\bd \to K^+ \pi^-}}
\newcommand{\abdkpi}{\ensuremath{\abd \to K^- \pi^+}}
\newcommand{\DCSbdkpi}{\ensuremath{\bd \to K^- \pi^+}}
\newcommand{\DCSabdkpi}{\ensuremath{\abd \to K^+ \pi^-}}
\newcommand{\DCSbskpi}{\ensuremath{\bs \to K^+ \pi^-}}
\newcommand{\DCSabskpi}{\ensuremath{\abs \to K^- \pi^+}}


\newcommand{\bskpi}{\ensuremath{\bs \to K^- \pi^+}}
\newcommand{\abskpi}{\ensuremath{\abs\to K^+ \pi^-}}
     
\newcommand{\bskk}{\ensuremath{\bs \to  K^+ K^-}}
\newcommand{\abskk}{\ensuremath{\abs \to  K^+ K^-}}
\newcommand{\bothbskk}{\ensuremath{\bs, \abs \to  K^+ K^-}}

\newcommand{\bspipi}{\ensuremath{\bs \to  \pi^+ \pi^-}}
\newcommand{\abspipi}{\ensuremath{\abs \to  \pi^+ \pi^-}}
\newcommand{\bothbspipi}{\ensuremath{\bs, \abs \to  \pi^+ \pi^-}}

\newcommand{\bdkk}{\ensuremath{\bd \to  K^+ K^-}}
\newcommand{\abdkk}{\ensuremath{\abd \to  K^+ K^-}}
\newcommand{\bothbdkk}{\ensuremath{\bd, \abd \to  K^+ K^-}}

\newcommand{\bnkk}{\ensuremath{\bn \to  K^+ K^-}}
\newcommand{\bnpipi}{\ensuremath{\bn \to  \pi^+ \pi^-}}

\newcommand{\bdpi}{\ensuremath{\bn \to  D^-_{(s)} \pi^+}}

\newcommand{\bddpi}{\ensuremath{\bd \to  \dminus \pi^+}}
\newcommand{\fullbddpi}{\ensuremath{\bd \to  \dminus \pi^+ \to [K^+ \pi^- \pi^-] \pi^+}}

\newcommand{\budzeropi}{\ensuremath{\bu \to  \adzero \pi^+}}

\newcommand{\bsdspi}{\ensuremath{\bs \to  \dsminus \pi^+}}
\newcommand{\fullbsdspi}{\ensuremath{\bs \to  \dsminus \pi^+ \to [\phi \pi^-]\pi^+ \to [[K^+ K^-]\pi^-] \pi^+}}
\newcommand{\extrafullbsdspi}{\ensuremath{\bs \to \dsminus \pi^+ \to [\phi(1020) \pi^-]\pi^+ \to [[K^+ K^-]\pi^-] \pi^+}}

\newcommand{\bjpsix}{\ensuremath{\bn \to  \jpsi X}}

\newcommand{\bdjpsikstar}{\ensuremath{\bd \to  \jpsi K^{*0}}}
\newcommand{\fullbdjpsikstar}{\ensuremath{\bd \to  \jpsi K^{*0} \to [\mu^+ \mu^-][K^+ \pi^-]}}
\newcommand{\extrafullbdjpsikstar}{\ensuremath{\bd \to  \jpsi K^{*}(892)^{0} \to [\mu^+ \mu^-][K^+ \pi^-]}}

\newcommand{\bujpsikplus}{\ensuremath{\bu \to  \jpsi K^{+}}}
\newcommand{\bujpsikminus}{\ensuremath{B^- \to  \jpsi K^{-}}}


\newcommand{\bsjpsiphi}{\ensuremath{\bs \to  \jpsi \phi}}
\newcommand{\fullbsjpsiphi}{\ensuremath{\bs \to  \jpsi \phi \to [\mu^+ \mu^-][K^+ K^-]}}
\newcommand{\extrafullbsjpsiphi}{\ensuremath{\bs \to  \jpsi \phi(1020) \to [\mu^+ \mu^-][K^+ K^-]}}

\newcommand{\lambdabppi}{\ensuremath{\lambdab \to \proton \pi^{-}}}
\newcommand{\lambdabpk}{\ensuremath{\lambdab \to \proton K^{-}}}


\newcommand{\deltagammas}{\ensuremath{\Delta\Gamma_s}}
\newcommand{\deltagammad}{\ensuremath{\Delta\Gamma_d}}
\newcommand{\dgogs}{\ensuremath{\deltagammas/\Gamma_s}}
\newcommand{\dgogd}{\ensuremath{\deltagammad/\Gamma_d}}



%	** CHARM **

\newcommand{\cac}{\ensuremath{c\bar{c}}}

%	** hadrons **

\newcommand{\jpsi}{\ensuremath{J/\psi}}

\newcommand{\cquark}{\mbox{$c$-quark}}    
\newcommand{\cquarks}{\mbox{$c$-quarks}}  

\newcommand{\squark}{\mbox{$s$-quark}}    
\newcommand{\squarks}{\mbox{$s$-quarks}}  
					  
\newcommand{\chadron}{\mbox{$c$-hadron}}  
\newcommand{\chadrons}{\mbox{$c$-hadrons}}

\newcommand{\dzero}{\ensuremath{D^{0}}}
\newcommand{\adzero}{\ensuremath{\overline{D}^{0}}}

\newcommand{\dminus}{\ensuremath{D^{-}}} 		  % D minus
\newcommand{\dsminus}{\ensuremath{D^{-}_s}}		  % D (minus) sub-s

\newcommand{\dplus}{\ensuremath{D^{+}}} 		  % D minus
\newcommand{\dsplus}{\ensuremath{D^{+}_s}}		  % D (minus) sub-s

\newcommand{\dstarplus}{\ensuremath{D^{*+}}} 		  % D star plus
\newcommand{\dstarminus}{\ensuremath{D^{*-}}}		  % D star minus

\newcommand{\dstarplusmeson}{\mbox{$D^{*+}$ meson}} 		  % D star plus
\newcommand{\dstarminusmeson}{\mbox{$D^{*-}$ meson}}		  % D star minus

\newcommand{\dstarplusmesons}{\mbox{$D^{*+}$ mesons}} 		  % D star plus
\newcommand{\dstarminusmesons}{\mbox{$D^{*-}$ mesons}}		  % D star minus



\newcommand{\dg}{\ensuremath{D}} 		  % D generic (neutral and charged)
\newcommand{\dgmeson}{\mbox{$c$-meson}}  	  % D generic (neutral and charged)
\newcommand{\dgmesons}{\mbox{$c$-mesons}}	  % D generic (neutral and charged)

\newcommand{\dcminus}{\ensuremath{D^{-}_{(s)}}}	  % D charged minus (D- and D-_s)
\newcommand{\dcmmeson}{\mbox{\dcminus\ meson}}	  % D charged minus (D- and D-_s)
\newcommand{\dcmmesons}{\mbox{\dcminus\ mesons}}  % D charged minus (D- and D-_s)

\newcommand{\dcplus}{\ensuremath{D^{+}_{(s)}}}	  % D charged plus (D+ and D+_s)
\newcommand{\dcpmeson}{\mbox{\dcplus\ meson}}	  % D charged plus (D+ and D+_s)
\newcommand{\dcpmesons}{\mbox{\dcplus\ mesons}}   % D charged plus (D+ and D+_s)

%	** decays **

								 
\newcommand{\dzerohh}{\ensuremath{\dzero \to h^+ h^{'-}}}

\newcommand{\dzerokpi}{\ensuremath{\dzero \to K^- \pi^+}}
\newcommand{\DCSdzerokpi}{\ensuremath{\dzero \to K^+ \pi^-}}

\newcommand{\adzerokpi}{\ensuremath{\adzero \to K^+ \pi^-}}

\newcommand{\dzeropipi}{\ensuremath{\dzero \to \pi^+ \pi^-}}
\newcommand{\dzerokk}{\ensuremath{\dzero \to K^+ K^-}}

\newcommand{\dpluskpipi}{\ensuremath{\dplus \to K^- \pi^+ \pi^+}}
\newcommand{\dminuskpipi}{\ensuremath{\dminus \to K^+ \pi^- \pi^-}}
\newcommand{\dpluskkpi}{\ensuremath{\dplus \to K^+ K^- \pi^+}}

\newcommand{\dspluskkpi}{\ensuremath{\dsplus \to K^+ K^- \pi^+}}
\newcommand{\dsminuskkpi}{\ensuremath{\dsminus \to K^+ K^- \pi^-}}

\newcommand{\dstarplusdzeropi}{\ensuremath{\dstarplus \to \dzero \pi^+}}

\newcommand{\fulldstarplus}{\ensuremath{\dstarplus \to \dzero \pi^+ \to [K^- \pi^+] \pi^+}}
\newcommand{\extrafulldstarplus}{\ensuremath{D^{*}(2010)^{+} \to \dzero \pi^+ \to [K^- \pi^+] \pi^+}}
\newcommand{\fulldstarminus}{\ensuremath{\dstarminus \to \adzero \pi^- \to [K^+ \pi^-] \pi^-}}

\newcommand{\bplusantidzeropi}{\ensuremath{\Bu \to \pi^+ \adzero}}


\newcommand{\dstardzerokpi}{\ensuremath{\dstarplus \to \dzero \pi^+ \to [K^- \pi^+] \pi^+}}
\newcommand{\dstardzeropipi}{\ensuremath{\dstarplus \to \dzero \pi^+ \to [\pi^+ \pi^-] \pi^+}}
\newcommand{\dstardzerokk}{\ensuremath{\dstarplus \to \dzero \pi^+ \to [K^+ K^-] \pi^+}}




%%%%%%%%%%%%%%%%% TEX CITATIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tesi}{thesis}

\newcommand{\page}[1]{pag.~\pageref{pag:#1}}

\newcommand{\figura}{figure}

%%% da usare dopo il punto.
\newcommand{\Fig}[1]{Figure \ref{fig:#1}}
\newcommand{\twoFig}[2]{Figures \ref{fig:#1} and \ref{fig:#2}}
\newcommand{\Figs}[2]{Figures \ref{fig:#1}--\ref{fig:#2}}
\newcommand{\Figindex}[2]{Figure \ref{fig:#1}(#2)}
\newcommand{\twoFigindex}[3]{Figures \ref{fig:#1}(#2) and (#3)}
\newcommand{\Figsindex}[3]{Figures \ref{fig:#1}(#2)--\ref{fig:#1}(#3)}

%da usare nel testo
\newcommand{\fig}[1]{fig.~\ref{fig:#1}}
\newcommand{\twofig}[2]{figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figs}[2]{figs.~\ref{fig:#1}--\ref{fig:#2}}
\newcommand{\figindex}[2]{fig.~\ref{fig:#1}(#2)}
\newcommand{\twofigindex}[3]{figs.~\ref{fig:#1}(#2) and (#3)}
\newcommand{\figsindex}[3]{figs.~\ref{fig:#1}(#2)--\ref{fig:#1}(#3)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tabella}{table}

%%% da usare dopo il punto.
\newcommand{\Tab}[1]{Table \ref{tab:#1}}
\newcommand{\twoTabs}[2]{Tables \ref{tab:#1} and \ref{tab:#2}}
\newcommand{\Tabs}[2]{Tables \ref{tab:#1}--\ref{tab:#2}}

%%% da usare nel testo.
\newcommand{\tab}[1]{tab.~\ref{tab:#1}}
\newcommand{\twotabs}[2]{tabs.~\ref{tab:#1} and \ref{tab:#2}}
\newcommand{\tabs}[2]{tabs.~\ref{tab:#1}--\ref{tab:#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\equazione}{equation}
\newcommand{\equazioni}{equations}

%%% da usare dopo il punto.
\newcommand{\Eq}[1]{Equation (\ref{eq:#1})}
\newcommand{\twoEqs}[2]{Equations (\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\Eqs}[2]{Equations (\ref{eq:#1})--(\ref{eq:#2})}
%%% da usare nel testo
\newcommand{\eq}[1]{eq.~(\ref{eq:#1})}
\newcommand{\twoeqs}[2]{eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\eqs}[2]{eqs.~(\ref{eq:#1})--(\ref{eq:#2})}

\newcommand{\se}[1]{system (\ref{eq:#1})}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% da usare dopo il punto.

\newcommand{\Rel}[1]{Relation (\ref{eq:#1})}
\newcommand{\twoRel}[2]{Relations (\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\Rels}[2]{Relations (\ref{eq:#1})--(\ref{eq:#2})}

%%% da usare nel testo

\newcommand{\rel}[1]{relation (\ref{eq:#1})}
\newcommand{\tworel}[2]{relations (\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\rels}[2]{relations (\ref{eq:#1})--(\ref{eq:#2})}

\newcommand{\capitolo}{chapter}
\newcommand{\capitoli}{chapters}
\newcommand{\chapt}[1]{chap.~\ref{chapt:#1}}	
\newcommand{\appdx}[1]{appendix \ref{appdx:#1}}
\newcommand{\Chapt}[1]{Chapter \ref{chapt:#1}}	
\newcommand{\Appdx}[1]{Appendix \ref{appdx:#1}}
\newcommand{\appendice}{appendix}
\newcommand{\appendici}{appendices}

\newcommand{\sezione}{section}
\newcommand{\sezioni}{sections}
\newcommand{\sect}[1]{sec.~\ref{sec:#1}}
\newcommand{\twosect}[2]{sec.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\sects}[2]{sec.~\ref{sec:#1}--\ref{sec:#2}}

%%% da usare dopo il punto.

\newcommand{\Sect}[1]{Section \ref{sec:#1}}
\newcommand{\twoSect}[2]{Sections \ref{sec:#1} and \ref{sec:#2}}
\newcommand{\Sects}[2]{Sections \ref{sec:#1}--\ref{sec:#2}}

%\newcommand{\ssect}[1]{Sec.\ \ref{ssec:#1}}
%\newcommand{\sssect}[1]{Sec.\ \ref{sssec:#1}}

\newcommand{\refcita}[1]{Ref.~\cite{#1}}
\newcommand{\refcitadue}[2]{Refs.~\cite{#1,#2}}
\newcommand{\refcitatre}[3]{Refs.~\cite{#1,#2,#3}}
\newcommand{\refcitaquattro}[4]{Refs.~\cite{#1,#2,#3,#4}}
\newcommand{\refcitacinque}[5]{Refs.~\cite{#1,#2,#3,#4,#5}}

%\newcommand{\refcitarange}[2]{Refs.\ \cite{#1,#2}}

\newcommand{\cita}[1]{\cite{#1}}
\newcommand{\citadue}[2]{\cite{#1,#2}}
\newcommand{\citatre}[3]{\cite{#1,#2,#3}}
\newcommand{\citaquattro}[4]{\cite{#1,#2,#3,#4}}
\newcommand{\citacinque}[5]{\cite{#1,#2,#3,#4,#5}}

%\newcommand{\citarange}[2]{Refs.\ \cite{#1,#2}}



%%%%%%%%%%%%%%%%% MY THESIS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\fracdedx}{\ensuremath{\frac{\mathit{dE}}{\mathit{dx}}}}
\newcommand{\fracdedxprime}{\ensuremath{\frac{\mathit{dE'}}{\mathit{dx'}}}}
\newcommand{\fracdedxsecond}{\ensuremath{\frac{\mathit{dE''}}{\mathit{dx''}}}}
\newcommand{\fracdedxn}{\ensuremath{\frac{\mathit{dE^n}}{\mathit{dx^n}}}}


\newcommand{\dedx}{\ensuremath{\mathit{dE/dx}}}
\newcommand{\dedxprime}{\ensuremath{\mathit{dE'/dx'}}}
\newcommand{\dedxsecond}{\ensuremath{\mathit{dE''/dx''}}}
\newcommand{\dedxn}{\ensuremath{\mathit{dE^n/dx^n}}}
\newcommand{\like}{\ensuremath{\mathscr{L}}}
\newcommand{\gauss}{\ensuremath{\mathscr{G}}}
\newcommand{\tail}{\ensuremath{\mathscr{T}}}
\newcommand{\argus}{\ensuremath{\mathscr{A}}}
\newcommand{\pdf}{\ensuremath{\wp}}
\newcommand{\ptot}{\ensuremath{p_{\rm{tot}}}}
\newcommand{\res}{\ensuremath{\delta}}
\newcommand{\id}{\ensuremath{\kappa}}
\newcommand{\nhit}{\ensuremath{\mathscr{N}}}
\newcommand{\sumpt}{\ensuremath{\sum\pt}}
\newcommand{\chitred}{\ensuremath{\chi^{2}_{3D}}}
\newcommand{\chitredB}{\ensuremath{\chi^{2}_{3D}(B)}}

\newcommand{\acpbdkpi}{\ensuremath{\acp(\bdkpi)}}		      
\newcommand{\pipisukpi}{\ensuremath{\br(\bdpipi)/\br(\bdkpi)}}
\newcommand{\kksukpi}{\ensuremath{(\mathit{f_s}/\mathit{f_d})\times\br(\bskk)/\br(\bdkpi)}}
\newcommand{\pipisukk}{\ensuremath{(\mathit{f_d}/\mathit{f_s})\times\br(\bdpipi)/\br(\bskk)}}
\newcommand{\ppisupk}{\ensuremath{\br(\Lbppi)/\br(\LbpK)}}
\newcommand{\limbskpi}{\ensuremath{(\mathit{f_s}/\mathit{f_d})\times\br(\bskpi)/\br(\bdkpi)}}
\newcommand{\limbspipi}{\ensuremath{\br(\bspipi)/\br(\bskk)}}
\newcommand{\limbdkk}{\ensuremath{\br(\bdkk)/\br(\bdkpi)}}

\newcommand{\fracacp}{\ensuremath{\frac{\br(\abdkpi) -\br(\bdkpi)}{\br(\abdkpi) +\br(\bdkpi)}}}
\newcommand{\fracpipisukpi}{\ensuremath{\frac{\br(\bdpipi)}{\br(\bdkpi)}}}
\newcommand{\frackksukpi}{\ensuremath{\frac{\mathit{f_s}}{\mathit{f_d}}\times\frac{\br(\bskk)}{\br(\bdkpi)}}}
\newcommand{\fracpipisukk}{\ensuremath{\frac{\mathit{f_d}}{\mathit{f_s}}\times\frac{\br(\bdpipi)}{\br(\bskk)}}}
\newcommand{\fraclimbskpi}{\ensuremath{\frac{\mathit{f_s}}{\mathit{f_d}}\times\frac{\br(\bskpi)}{\br(\bdkpi)}}}
\newcommand{\fraclimbspipi}{\ensuremath{\frac{\br(\bspipi)}{\br(\bskk)}}}
\newcommand{\fraclimbdkk}{\ensuremath{\frac{\br(\bdkk)}{\br(\bdkpi)}}}

\newcommand{\BRbdpipi}{\ensuremath{\br(\bdpipi)}}
\newcommand{\BRbdkpi}{\ensuremath{\br(\bdkpi)}}
\newcommand{\BRbskk}{\ensuremath{\br(\bskk)}}
\newcommand{\BRbspipi}{\ensuremath{\br(\bspipi)}}
\newcommand{\BRbskpi}{\ensuremath{\br(\bskpi)}}
\newcommand{\BRbdkk}{\ensuremath{\br(\bdkk)}}
\newcommand{\BRLbppi}{\ensuremath{\br(\Lbppi)}}
\newcommand{\BRLbpK}{\ensuremath{\br(\LbpK)}}



% BIBLIOGRAFIA STYLES AND ALIASES


\newcommand{\oneauthor}[1]{\textsc{#1},}
\newcommand{\twoauthors}[2]{\textsc{#1} and \textsc{#2},}
\newcommand{\threeauthors}[3]{\textsc{#1, #2,} and \textsc{#3},}
\newcommand{\fourauthors}[4]{\textsc{#1, #2, #3, \rm{and} #4},}
\newcommand{\fiveauthors}[5]{\textsc{#1, #2, #3, #4, \rm{and} #5},}
\newcommand{\manyauthors}[1]{\textsc{#1} \etal,}
%\newcommand{\collaboration}[2]{\textsc{#1} \etal\ \textsc{(#2 Collaboration)},}
\newcommand{\group}[2]{\textsc{#1} \etal\ \textsc{(#2 Group)},}
\newcommand{\conference}[2]{\textsc{#1} for the \textsc{#2 Collaboration},}
\newcommand{\paper}[1]{\newblock{\emph{#1}},}

\newcommand{\etal}{et al.}
\newcommand{\PRv}[3]{Phys.\ Rev.\ \textbf{#1}, #2 (#3)}
\newcommand{\PRL}[3]{Phys.\ Rev.\ Lett.\ \textbf{#1}, #2 (#3)}
\newcommand{\RMP}[3]{ Rev.\ Mod.\ Phys.\ \textbf{#1}, #2 (#3)}
\newcommand{\PRD}[3]{Phys.\ Rev.\ D \textbf{#1}, #2 (#3)}
\newcommand{\PLB}[3]{Phys.\ Lett.\  \textbf{B#1}, #2 (#3)}
\newcommand{\NIMA}[3]{Nucl.\ Instrum.\ Methods \textbf{A#1}, #2 (#3)}
\newcommand{\NIM}[2]{Nucl.\ Instrum.\ Methods #1 (#2)}
\newcommand{\NPB}[3]{Nucl.\ Phys.\ \textbf{B #1}, #2 (#3)}
\newcommand{\NPBproc}[3]{Nucl.\ Phys.\ \textbf{B} (Proc.\ Suppl.) \textbf{#1}, #2 (#3)}
\newcommand{\econf}[3]{eConf.\ \textbf{#1} #2 (#3)}
\newcommand{\cdfnote}[2]{CDF Internal Note #1 (#2), unpublished}
\newcommand{\cdfnotePUBLIC}[2]{CDF Internal Note #1 (#2), published}
\newcommand{\ieee}[3]{IEEE Trans.\ Nucl.\ Sci.\ \textbf{#1}, #2 (#3)}
\newcommand{\EPJ}[3]{Eur.\ Phys.\ J.\ \textbf{#1}, #2 (#3)}
\newcommand{\PR}[3]{Phys.\ Rept.\ \textbf{#1}, #2 (#3)}
\newcommand{\AR}[3]{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ \textbf{#1}, #2 (#3)}
\newcommand{\ZFC}[3]{Z.\ Phys.\ C \textbf{#1}, #2 (#3)}
\newcommand{\ZF}[3]{Z.\ Phys.\ \textbf{#1}, #2 (#3)}
\newcommand{\arxiv}[1]{\textsf{[#1]}}
%\newcommand{\oneauthor}[1]{\textrm{#1}}
%\newcommand{\twoauthors}[2]{\textrm{#1 and #2}}
%\newcommand{\threeauthors}[3]{\textrm{#1, #2, and #3}}
%\newcommand{\fourauthors}[4]{\textrm{#1, #2, #3, and #4}}
%\newcommand{\manyauthors}[1]{\textrm{#1 \etal}}
%\newcommand{\collaboration}[2]{\textrm{#1 \etal\ (#2 Collaboration)}}
%\newcommand{\paper}[1]{\newblock{\textrm{``#1''}}}
 
%\newcommand{\etal}{\emph{et al.\ }}
%\newcommand{\PRL}[3]{\emph{Phys.\ Rev.\ Lett.} \textbf{#1}, #2 (#3)}
%\newcommand{\PRD}[3]{\emph{Phys.\ Rev.\ D} \textbf{#1}, #2 (#3)}
%\newcommand{\PLB}[3]{\emph{Phys.\ Lett.\ B} \textbf{#1}, #2 (#3)}
%\newcommand{\NIMA}[3]{\emph{Nucl.\ Instrum.\ Methods\ Phys.\ Res.\ Sect.\ A}
% \textbf{#1}, #2 (#3)}
%\newcommand{\NPB}[3]{\emph{Nucl.\ Phys.} \textbf{B #1}, #2 (#3)}
%\newcommand{\econf}[3]{\emph{eConf.} \textbf{#1} #2 (#3)}
%\newcommand{\cdfnote}[2]{\emph{CDF Internal Note #1 (#2)}, unpublished}
%\newcommand{\ieee}[3]{\emph{IEEE Trans.\ Nucl.\ Sci.} \textbf{#1}, #2 (#3)}


\newcommand{\babar}{{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em}\sl B\hspace{-0.4em}}} {\small\sl A\hspace{-0.02em}R}}
\newcommand{\cleo}{CLEO}  
\newcommand{\belle}{Belle}



% Aggiunte Michael 
\newcommand{\Bhh}{\ensuremath{\bn \rightarrow h^{+}h^{'-}}}
\newcommand{\Bdhh}{\ensuremath{\bd \rightarrow h^{+}h^{'-}}}
\newcommand{\Bshh}{\ensuremath{\bs \rightarrow h^{+}h^{'-}}}
\newcommand{\Lbph}{\ensuremath{\Lambda^{0}_{b} \rightarrow ph^{-}}}
\newcommand{\Bnrhopi}{\ensuremath{\bn \rightarrow \rho^{-}\pi^{+}}}
\newcommand{\Bdpipi}{\ensuremath{\bd \rightarrow \pi^+ \pi^-}}
\newcommand{\Bdpipic}{\ensuremath{\bd \rightarrow \pi^- \pi^+}}
\newcommand{\Bnpipi}{\ensuremath{\bn \rightarrow \pi^+ \pi^-}}
\newcommand{\aBdpipi}{\ensuremath{\overline{B}^{0} \rightarrow \pi^+ \pi^-}}
\newcommand{\BdKpi}{\ensuremath{\bd \rightarrow K^{+} \pi^-}}
\newcommand{\BdKpic}{\ensuremath{\bd \rightarrow \pi^- K^{+}}}
\newcommand{\aBdKpi}{\ensuremath{\abd \rightarrow K^- \pi^+}}
\newcommand{\aBdKpic}{\ensuremath{\abd \rightarrow \pi^+ K^-}}
\newcommand{\BsKpi}{\ensuremath{\bs \rightarrow K^- \pi^+}}
\newcommand{\BsKpic}{\ensuremath{\bs \rightarrow \pi^+ K^-}}
\newcommand{\aBsKpi}{\ensuremath{\abs\rightarrow K^+ \pi^-}}
\newcommand{\aBsKpic}{\ensuremath{\abs\rightarrow \pi^- K^+}}
\newcommand{\BsKK}{\ensuremath{\bs \rightarrow  K^+ K^-}}
\newcommand{\BsKKc}{\ensuremath{\bs \rightarrow  K^- K^+}}
\newcommand{\BnKK}{\ensuremath{\bn \rightarrow  K^+ K^-}}
\newcommand{\aBsKK}{\ensuremath{\overline{B}^{0}_{s} \rightarrow  K^+ K^-}}
\newcommand{\Bspipi}{\ensuremath{\bs \rightarrow  \pi^+ \pi^-}}
\newcommand{\Bspipic}{\ensuremath{\bs \rightarrow  \pi^- \pi^+}}
\newcommand{\aBspipi}{\ensuremath{\overline{B}^{0}_{s} \rightarrow  \pi^+ \pi^-}}
\newcommand{\BdKK}{\ensuremath{\bd \rightarrow  K^+ K^-}}
\newcommand{\BdKKc}{\ensuremath{\bd \rightarrow  K^- K^+}}
\newcommand{\aBdKK}{\ensuremath{\overline{B}^0 \rightarrow  K^+ K^-}}
\newcommand{\Lbppi}{\ensuremath{\Lambda_{b}^{0} \rightarrow p\pi^{-}}}
\newcommand{\Lbppic}{\ensuremath{\Lambda_{b}^{0} \rightarrow \pi^{-}p}}
\newcommand{\aLbppi}{\ensuremath{\overline{\Lambda}_{b}^{0} \rightarrow \overline{p}\pi^{+}}}
\newcommand{\aLbppic}{\ensuremath{\overline{\Lambda}_{b}^{0} \rightarrow \pi^{+}\overline{p}}}
\newcommand{\Lppi}{\ensuremath{\Lambda^{0} \rightarrow p\pi^{-}}}
\newcommand{\Lppic}{\ensuremath{\Lambda^{0} \rightarrow \pi^{-}p}}
\newcommand{\aLppi}{\ensuremath{\overline{\Lambda}^{0} \rightarrow \overline{p}\pi^{+}}}
\newcommand{\aLppic}{\ensuremath{\overline{\Lambda}^{0} \rightarrow \pi^{+}\overline{p}}}
\newcommand{\LbpK}{\ensuremath{\Lambda_{b}^{0} \rightarrow pK^{-}}}
\newcommand{\LbpKc}{\ensuremath{\Lambda_{b}^{0} \rightarrow K^{-}p}}
\newcommand{\aLbpK}{\ensuremath{\overline{\Lambda}_{b}^{0} \rightarrow \overline{p}K^{+}}}
\newcommand{\aLbpKc}{\ensuremath{\overline{\Lambda}_{b}^{0} \rightarrow K^{+}\overline{p}}}


\newcommand{\Bdrhopi}{\ensuremath{B^0 \rightarrow \rho^{\mp}\pi^{\pm}}}
\newcommand{\Bsrhopi}{\ensuremath{B^0_s \rightarrow \rho^{\mp}\pi^{\pm}}}
\newcommand{\Burhopi}{\ensuremath{B^+ \rightarrow \rho^{-}\pi^{+}}}

\newcommand{\BdrhoK}{\ensuremath{B^0 \rightarrow \rho^{-}K^{+}}}
\newcommand{\BsrhoK}{\ensuremath{B^0_s \rightarrow \rho^{+}K^{-}}}
\newcommand{\BurhoK}{\ensuremath{B^+ \rightarrow \rho^{0}K^{+}}}

\newcommand{\Bdhhh}{\ensuremath{B^0   \rightarrow h_{1}^{+} h_{2}^{-} h_{3}^{0}}}
\newcommand{\Buhhh}{\ensuremath{B^+   \rightarrow h_{1}^{+} h_{2}^{-} h_{3}^{+}}}
\newcommand{\Bshhh}{\ensuremath{B^0_s \rightarrow h_{1}^{+} h_{2}^{-} h_{3}^{0}}}


\newcommand{\BuKpi}{\ensuremath{\bu \rightarrow K^{+} \pi^0}}

%ACP raw
\newcommand{\acpBdKpiRAW}{\ensuremath{\frac{\hat{f}_{\aBdKpi}~-~\hat{f}_{\BdKpi}}{\hat{f}_{\aBdKpi}~+~\hat{f}_{\BdKpi}}}}  
\newcommand{\acpBsKpiRAW}{\ensuremath{\frac{\hat{f}_{\aBsKpi}~-~\hat{f}_{\BsKpi}}{\hat{f}_{\aBsKpi}~+~\hat{f}_{\BsKpi}}}}  
\newcommand{\acpLbppiRAW}{\ensuremath{\frac{\hat{f}_{\aLbppi}~-~\hat{f}_{\Lbppi}}{\hat{f}_{\aLbppi}~+~\hat{f}_{\Lbppi}}}}  
\newcommand{\acpLbpKRAW}{\ensuremath{\frac{\hat{f}_{\aLbpK}~-~\hat{f}_{\LbpK}}{\hat{f}_{\aLbpK}~+~\hat{f}_{\LbpK}}}}  
\newcommand{\acpDKpiRAW}{\ensuremath{\frac{\hat{f}_{\aDKpi}~-~\hat{f}_{\DKpi}}{\hat{f}_{\aDKpi}~+~\hat{f}_{\DKpi}}}}  

\newcommand{\acpBdKpiRAWs}{\ensuremath{\hat{{\cal A}}_{\CP}(\BdKpi)}}  
\newcommand{\acpBsKpiRAWs}{\ensuremath{\hat{{\cal A}}_{\CP}(\BsKpi)}}  
\newcommand{\acpLbppiRAWs}{\ensuremath{\hat{{\cal A}}_{\CP}(\Lbppi)}}   
\newcommand{\acpLbpKRAWs}{\ensuremath{\hat{{\cal A}}_{\CP}(\LbpK)}}  
\newcommand{\acpDKpiRAWs}{\ensuremath{\hat{{\cal A}}_{\CP}(\DKpi)}}  



% altre osservabili raw
\newcommand{\ratioRAW}{\ensuremath{\frac{\hat{f}_{\aBdKpi}~-~\hat{f}_{\BdKpi}}{\hat{f}_{\aBsKpi}~+~\hat{f}_{\BsKpi}}}}
\newcommand{\BsKpisuBdKpiRAW}{\ensuremath{\frac{\hat{f}_{\BsKpi}}{\hat{f}_{\BdKpi}}}}
\newcommand{\BdpipisuBdKpiRAW}{\ensuremath{\frac{\hat{f}_{\Bdpipi}}{\hat{f}_{\BdKpi}}}}
\newcommand{\BsKKsuBdKpiRAW}{\ensuremath{\frac{\hat{f}_{\BsKK}}{\hat{f}_{\BdKpi}}}}
\newcommand{\BspipisuBdKpiRAW}{\ensuremath{\frac{\hat{f}_{\Bspipi}}{\hat{f}_{\BdKpi}}}}
\newcommand{\BdKKsuBdKpiRAW}{\ensuremath{\frac{\hat{f}_{\BdKK}}{\hat{f}_{\BdKpi}}}}
\newcommand{\LbpKsuBdKpiRAW}{\ensuremath{\frac{\hat{f}_{\LbpK}}{\hat{f}_{\BdKpi}}}}
\newcommand{\LbppisuBdKpiRAW}{\ensuremath{\frac{\hat{f}_{\Lbppi}}{\hat{f}_{\BdKpi}}}}
\newcommand{\LbppisuLbpKRAW}{\ensuremath{\frac{\hat{f}_{\Lbppi}}{\hat{f}_{\LbpK}}}}


\newcommand{\bhha}{\ensuremath{\bn \rightarrow hh}}
\newcommand{\bdpipia}{\ensuremath{\bd \rightarrow \pi\pi}}
\newcommand{\bdkpia}{\ensuremath{\bd \rightarrow K\pi}}
\newcommand{\abdkpia}{\ensuremath{\abd \rightarrow K\pi}}
\newcommand{\bskpia}{\ensuremath{\bs \rightarrow K \pi}}
\newcommand{\abskpia}{\ensuremath{\abs\rightarrow K \pi}}
\newcommand{\bskka}{\ensuremath{\bs \rightarrow  K K}}
\newcommand{\bspipia}{\ensuremath{\bs \rightarrow  \pi\pi}}
\newcommand{\bdkka}{\ensuremath{\bd \rightarrow  KK}}
\newcommand{\Lbppia}{\ensuremath{\Lambda_{b}^{0} \rightarrow p\pi}}
\newcommand{\aLbppia}{\ensuremath{\overline{\Lambda}_{b}^{0} \rightarrow \overline{p}\pi}}
\newcommand{\LbpKa}{\ensuremath{\Lambda_{b}^{0} \rightarrow pK}}
\newcommand{\aLbpKa}{\ensuremath{\overline{\Lambda}_{b}^{0} \rightarrow \overline{p}}}



\newcommand{\BR}{\ensuremath{\mathcal B}}

%osservabili
\newcommand{\ACPddef}{\ensuremath{{\frac{\BR (\aBdKpi)-\BR 
(\BdKpi)}{\BR (\aBdKpi)+\BR (\BdKpi)}}}}
\newcommand{\ACPsdef}{\ensuremath{{\frac{\BR (\aBsKpi)-\BR 
(\BsKpi)}{\BR (\aBsKpi)+\BR (\BsKpi)}}}}
\newcommand{\rateratiodef}{\ensuremath{\frac{\mathit{f_d}}{\mathit{f_s}}\times{\frac{\Gamma (\aBdKpi)-\Gamma 
(\BdKpi)}{\Gamma (\aBsKpi)-\Gamma (\BsKpi)}}}}
\newcommand{\rateratiodefNOfsfd}{\ensuremath{{\frac{\Gamma (\aBdKpi)-\Gamma 
(\BdKpi)}{\Gamma (\aBsKpi)-\Gamma (\BsKpi)}}}}


\newcommand{\BdpipisuBdKpidef}{\ensuremath{\frac{\BR(\Bdpipi)}{\BR(\BdKpi)}}}
\newcommand{\BsKKsuBdKpidef}{\ensuremath{\frac{\mathit{f_s}}{\mathit{f_d}}\times \frac{\BR(\BsKK)}{\BR(\BdKpi)}}}
\newcommand{\BdpipisuBsKKdef}{\ensuremath{\frac{\mathit{f_d}}{\mathit{f_s}}\times\frac{\BR(\Bspipi)}{\BR(\BsKK)}}}
\newcommand{\BsKpisuBdKpidef}{\ensuremath{\frac{\mathit{f_s}}{\mathit{f_d}}\times\frac{\BR(\BsKpi)}{\BR(\BdKpi)}}}
\newcommand{\BspipisuBdKpidef}{\ensuremath{\frac{\mathit{f_s}}{\mathit{f_d}}\times\frac{\BR(\Bspipi)}{\BR(\BdKpi)}}}
\newcommand{\BdKKsuBdKpidef}{\ensuremath{\frac{\BR(\BdKK)}{\BR(\BdKpi)}}}

\newcommand{\LbppisuBdKpidef}{\ensuremath{\frac{\mathit{f_{\Lambda}}}{\mathit{f_d}}\frac{\BR(\Lbppi)}{\BR(\BdKpi)}}}
\newcommand{\LbpKsuBdKpidef}{\ensuremath{\frac{\mathit{f_{\Lambda}}}{\mathit{f_d}}\frac{\BR(\LbpK)}{\BR(\BdKpi)}}}
\newcommand{\LbppisuLbpKdef}{\ensuremath{\frac{\BR(\Lbppi)}{\BR(\LbpK)}}}

\newcommand{\ACPdzerodef}{\ensuremath{{\frac{\BR (\aDKpi)-\BR (\DKpi)}{\BR (\aDKpi)+\BR (\DKpi)}}}}


%%%%%%%%%%%%%%%%%%% Mattias %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\nn{\nonumber}
\def\sss{\scriptscriptstyle}
%\def\bd{B_d^0}
\def\bdbar{{\overline{B_d^0}}}
%\def\bs{B_s^0}
\def\bsbar{{\overline{B_s^0}}}
\def\barp{{\raise.35ex\hbox
{${\sss (}$}}---{\raise.35ex\hbox{${\sss )}$}}}
\def\bdbarp{\hbox{$B_d$\kern-1.4em\raise1.4ex\hbox{\barp}}}
\def\bsbarp{\hbox{$B_s$\kern-1.4em\raise1.4ex\hbox{\barp}}}
\def\ks{K_{\sss S}}
\def\kbar{{\overline{K^0}}}
\def\roughly#1{\mathrel{\raise.3ex\hbox
{$#1$\kern-.75em\lower1ex\hbox{$\sim$}}}}
\def\lsim{\roughly<}
\def\gsim{\roughly>}
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\pew{P_{\sss EW}}
\def\pewc{P_{\sss EW}^{\sss C}}
\def\pewcp{P_{\sss EW}^{\prime \sss C}}
% Journal and other miscellaneous abbreviations for references
\def\epjc#1#2#3{{ Eur.\ Phys.\ J.}\ {\bf C#1}, #3, (#2)}
\def\ijmp#1#2#3{{ Int.\ J.\ Mod.\ Phys.} {\bf A#1}, #3 (#2)}
\def\mpla#1#2#3{{Mod.\ Phys.\ Lett.} {\bf A#1}, #3 (#2)}
\def\nci#1#2#3{{ Nuovo Cimento} {\bf #1}, #3 (#2)}
\def\npb#1#2#3{{ Nucl.\ Phys.} {\bf B#1}, #3 (#2)}
\def\plb#1#2#3{{ Phys.\ Lett.} {\bf #1B}, #3 (#2)}
\def\prd#1#2#3{{ Phys.\ Rev.} {\bf D#1}, #3 (#2)}
\def\prl#1#2#3{{ Phys.\ Rev.\ Lett.} {\bf #1}, #3 (#2)}
\def\zpc#1#2#3{{ Zeit.\ Phys.} {\bf C#1}, #3 (#2)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%giordano
%\newcommand{\ket}[1]{\left| #1 \right\rangle}
%\newcommand{\bra}[1]{\left\langle #1 \right|}
\newcommand{\CPp}{\textsf{CP}-parit\`a\ }


\newcommand{\Lxy}{\ensuremath{L_{\rm{T}}}}			%	Lxy
\newcommand{\phizero}{\ensuremath{\varphi_{0}}}			%	phi0
%\newcommand{\dzero}{\ensuremath{d_{0}}}                            %	d0

%\newcommand{\acpbdkpi}{\ensuremath{A_{\mathsf{CP}}(\bdkpi)}}
\newcommand{\acpbskpi}{\ensuremath{\acp(\bskpi)}}
\newcommand{\acpLbppi}{\ensuremath{\acp(\Lbppi)}}
\newcommand{\acpLbpK}{\ensuremath{ \acp(\LbpK)}}

\newcommand{\acpDKpi}{\ensuremath{\acp(\DKpi)}}
		      
%\newcommand{\pipisukpi}{\ensuremath{\mathcal{B}(\bdpipi)/\mathcal{B}(\bdkpi)}}
%\newcommand{\kksukpi}{\ensuremath{(\mathit{f_s}/\mathit{f_d})\cdot\mathcal{B}(\bskk)/\mathcal{B}(\bdkpi)}}
%\newcommand{\pipisukk}{\ensuremath{(\mathit{f_d}/\mathit{f_s})\cdot\mathcal{B}(\bdpipi)/\mathcal{B}(\bskk)}}
\newcommand{\bskpisubdkpi}{\ensuremath{(\mathit{f_s}/\mathit{f_d})\times \mathcal{B}(\bskpi)/\mathcal{B}(\bdkpi)}}
\newcommand{\rateratio}{\ensuremath{(\mathit{f_d}/\mathit{f_s})\times (\Gamma(\abdkpi) - \Gamma(\bdkpi))/(\Gamma(\abskpi) - \Gamma(\bskpi))}}
\newcommand{\bspipisubdkpi}{\ensuremath{(\mathit{f_s}/\mathit{f_d})\times \mathcal{B}(\bspipi)/\mathcal{B}(\bdkpi)}}
\newcommand{\bdkksubdkpi}{\ensuremath{\mathcal{B}(\bdkk)/\mathcal{B}(\bdkpi)}}

\newcommand{\LbppisuBdKpi}{\ensuremath{\mathcal{B}(\Lbppi)/\mathcal{B}(\bdkpi)}}
\newcommand{\LbpKsuBdKpi}{\ensuremath{\mathcal{B}(\LbpK)/\mathcal{B}(\bdkpi)}}
\newcommand{\LbpKsuLbppi}{\ensuremath{\mathcal{B}(\LbpK)/\mathcal{B}(\Lbppi)}}
\newcommand{\LbppisuLbpK}{\ensuremath{\mathcal{B}(\Lbppi)/\mathcal{B}(\LbpK)}}

\newcommand{\Nbdkpi}{\ensuremath{\mathcal{N}(\BdKpi)}}
\newcommand{\Nbdpipi}{\ensuremath{\mathcal{N}(\Bdpipi)}}
\newcommand{\Nbdkk}{\ensuremath{\mathcal{N}(\BdKK)}}
\newcommand{\Nbskpi}{\ensuremath{\mathcal{N}(\BsKpi)}}
\newcommand{\Nbspipi}{\ensuremath{\mathcal{N}(\Bspipi)}}
\newcommand{\Nbskk}{\ensuremath{\mathcal{N}(\BsKK)}}
\newcommand{\NLbppi}{\ensuremath{\mathcal{N}(\Lbppi)}}
\newcommand{\NLbpK}{\ensuremath{\mathcal{N}(\LbpK)}}

\newcommand{\Nabdkpi}{\ensuremath{\mathcal{N}(\aBdKpi)}}
\newcommand{\Nabdpipi}{\ensuremath{\mathcal{N}(\aBdpipi)}}
\newcommand{\Nabdkk}{\ensuremath{\mathcal{N}(\aBdKK)}}
\newcommand{\Nabskpi}{\ensuremath{\mathcal{N}(\aBsKpi)}}
\newcommand{\Nabspipi}{\ensuremath{\mathcal{N}(\aBspipi)}}
\newcommand{\Nabskk}{\ensuremath{\mathcal{N}(\aBsKK)}}
\newcommand{\NaLbppi}{\ensuremath{\mathcal{N}(\aLbppi)}}
\newcommand{\NaLbpK}{\ensuremath{\mathcal{N}(\aLbpK)}}


\newcommand{\NDKpi}{\ensuremath{\mathcal{N}(\DKpi)}}
\newcommand{\NaDKpi}{\ensuremath{\mathcal{N}(\aDKpi)}}

%\newcommand{\limbskpi}{\ensuremath{(\mathit{f_s}/\mathit{f_d})\cdot\mathcal{B}(\bskpi)/\mathcal{B}(\bdkpi)}}
%\newcommand{\limbspipi}{\ensuremath{\mathcal{B}(\bspipi)/\mathcal{B}(\bskk)}}
%\newcommand{\limbdkk}{\ensuremath{\mathcal{B}(\bdkk)/\mathcal{B}(\bdkpi)}}


%\newcommand{\fracpipisukpi}{\ensuremath{\frac{\mathcal{B}(\bdpipi)}{\mathcal{B}(\bdkpi)}}}
%\newcommand{\frackksukpi}{\ensuremath{\frac{\mathit{f_s}}{\mathit{f_d}}\cdot\frac{\mathcal{B}(\bskk)}{\mathcal{B}(\bdkpi)}}}
%\newcommand{\fracpipisukk}{\ensuremath{\frac{\mathit{f_d}}{\mathit{f_s}}\cdot\frac{\mathcal{B}(\bdpipi)}{\mathcal{B}(\bskk)}}}
%\newcommand{\fraclimbskpi}{\ensuremath{\frac{\mathit{f_s}}{\mathit{f_d}}\cdot\frac{\mathcal{B}(\bskpi)}{\mathcal{B}(\bdkpi)}}}
%\newcommand{\fraclimbspipi}{\ensuremath{\frac{\mathcal{B}(\bspipi)}{\mathcal{B}(\bskk)}}}
%\newcommand{\fraclimbdkk}{\ensuremath{\frac{\mathcal{B}(\bdkk)}{\mathcal{B}(\bdkpi)}}}

%\newcommand{\BRbdpipi}{\ensuremath{\mathcal{B}(\bdpipi)}}
%\newcommand{\BRbskk}{\ensuremath{\mathcal{B}(\bskk)}}
%\newcommand{\BRbspipi}{\ensuremath{\mathcal{B}(\bspipi)}}
%\newcommand{\BRbskpi}{\ensuremath{\mathcal{B}(\bskpi)}}
%\newcommand{\BRbdkk}{\ensuremath{\mathcal{B}(\bdkk)}}


\newcommand{\Bd}{\ensuremath{B^{0}}}
\newcommand{\aBd}{\ensuremath{\overline{B}^{0}}}

\newcommand{\BBd}{\ensuremath{\overline{B}^{0}}}
\newcommand{\Bu}{\ensuremath{B^{+}}}
\newcommand{\Bs}{\ensuremath{B_{s}^{0}}}
\newcommand{\aBs}{\ensuremath{\overline{B}_{s}^{0}}}

\newcommand{\Lb}{\ensuremath{\Lambda_{b}^{0}}}


\newcommand{\no}{\nonumber}
\newcommand{\cO}{{\cal O}}
\newcommand{\cA}{{\cal A}}

%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
\newcommand{\bear}{\begin{array}}
\newcommand{\ear}{\end{array}}
\newcommand{\bet}{\begin{tabular}}
\newcommand{\eet}{\end{tabular}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}

%D0->hh
\newcommand{\Dpipi}{\ensuremath{D^{0} \rightarrow \pi^+ \pi^-}}
\newcommand{\Dkpi}{\ensuremath{D^{0} \rightarrow K^- \pi^+}}
\newcommand{\aDkpi}{\ensuremath{\overline{D}^{0} \rightarrow K^+ \pi^-}}
\newcommand{\Dkk}{\ensuremath{D^{0} \rightarrow K^+ K^-}}
\newcommand{\acpdkpi}{\ensuremath{A_{\mathsf{CP}}(\Dkpi)}}


\newcommand{\DKpi}{\ensuremath{D^{0} \rightarrow K^- \pi^+}}
\newcommand{\aDKpi}{\ensuremath{\overline{D}^{0} \rightarrow K^+ \pi^-}}
\newcommand{\DKK}{\ensuremath{D^{0} \rightarrow K^+ K^-}}



%%%%%%%%%%%%%%%%%%% Notazione Centro di Mass %%%%%%%


%\newcommand{\pCM}[1]{\ensuremath{\vec{p}^{~*}_{#1}}}
%\newcommand{\ptCM}[1]{\ensuremath{p^{*}_{T#1}}}
%\newcommand{\EnCM}[1]{\ensuremath{E^{*}_{#1}}}
%\newcommand{\EnCM}[1]{\ensuremath{E^{*}_{#1}}}

